Credit-Based vs. Discount-Based Congestion Pricing: A Comparison Study

Credit-based congestion pricing (CBCP) and discount-based congestion pricing (DBCP), which respectively allot travel credits and toll discounts to subsidize low-income users' access to tolled roads, have emerged as promising policies for alleviating the societal inequity concerns of congestion pricing. However, since real-world deployments of CBCP and DBCP remain limited, transportation agencies lack clear guidance on which policy better achieves travel cost reduction and revenue generation objectives. In this work, we compare the efficacy of deploying CBCP and DBCP in reducing user costs and increasing toll revenues. We first formulate a non-atomic congestion game in which low-income users receive a travel credit or toll discount for accessing tolled lanes. We establish that, in our formulation, Nash equilibrium flows always exist and can be computed or well approximated via convex programming. Our main result establishes a set of practically relevant conditions under which DBCP provably outperforms CBCP in inducing equilibrium outcomes that minimize a given societal cost, which encodes user cost reduction and toll revenue maximization. Finally, we validate our theoretical contributions via a case study of the 101 Express Lanes Project, a CBCP program implemented in the San Francisco Bay Area. Our results provide theoretical and computational foundations for evaluating equity-oriented congestion pricing policies and offer practical guidance for transportation agencies seeking to design congestion pricing programs that better balance travel cost reduction and revenue generation objectives.

==> temp_postdoctoral_research_symposium.tex <==
% temp_postdoctoral_research_symposium.tex

% % (Avg) lambda_R \geq \lambda_E; Express Lane usage and Average travel time

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|} 
    \hline
    Weights & Policy &
    \multicolumn{3}{c|}{Express Lane usage (\%)} & \multicolumn{2}{c|}{Avg travel time (min)} \\
    \cline{3-7}
    $(\lambda_E, \lambda_R, \lambda_I)$ & 
    % (CBCP or DBCP)
    & Overall & Eligible & Ineligible & \hspace{2mm} Express \hspace{2mm} & GP \\
    % & \multicolumn{2}{c|}{Total travel costs} & Total toll revenue \\
    % \multirow{3}{4em}{\centering o-d Node Indices} & \multicolumn{2}{c|}{o-d Cities} & \multicolumn{5}{c|}{Demand of group $g \in [5]$} \\
    % \cline{2-8}
    % & \multirow{2}{*}{Origin} & \multirow{2}{*}{Destination} & $g=1$ & $g=2$ & $g=3$ & $g=4$ & $g=5$ \\
    % & & & (El) & (El) & (Inel) & (Inel) & (Inel) \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(1, 5, 1)$} & CBCP & 16.34 & 32.51 & 13.08 & 21.17 & 25.21 \\
    \cline{2-7}
    & DBCP & 19.39 & 33.12 & 16.63 & 21.45 & 24.72 \\
    \hline
    \multirow{2}{*}{\centering $(5, 5, 1)$} & CBCP & 17.60 & 51.88 & 10.68 & 21.46 & 25.12 \\
    \cline{2-7}
    & DBCP & 19.64 & 38.87 & 15.77 & 21.79 & 24.64 \\
    \hline
    \multirow{2}{*}{\centering $(10, 10, 1)$} & CBCP & 15.22 & 45.56 & 9.09 & 20.95 & 25.34 \\
    \cline{2-7}
    & DBCP & 17.10 & 43.28 & 11.82 & 21.11 & 25.04 \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(5, 1, 1)$} & CBCP & 15.67 & 58.00 & 7.13 & 21.42 & 25.12 \\
    \cline{2-7}
    & DBCP & 23.46 & 40.68 & 19.98 & 23.14 & 24.07 \\
    \hline
    \multirow{2}{*}{\centering $(5, 1, 0)$} & CBCP & 14.46 & 47.84 & 7.71 & 21.11 & 25.43 \\
    \cline{2-7}
    & DBCP & 16.78 & 41.56 & 11.77 & 21.38 & 24.97 \\
    \hline
    \multirow{2}{*}{\centering $(20, 1, 0)$} & CBCP & 13.74 & 53.88 & 5.65 & 20.77 & 25.52 \\
    \cline{2-7}
    & DBCP & 18.73 & 57.30 & 10.95 & 21.22 & 24.95 \\
    \hline
    \end{tabular}
    \caption{
    (For the 2025 GT Postdoctoral Research Symposium)
    Average express lane usage and average travel time at equilibrium, under the optimal CBCP and DBCP policies with respect to a range of weight parameters $(\lambda_E, \lambda_R, \lambda_I)$.
    }
    % \label{Table: (Avg) Express Lane Usage and Average Travel Time, for lambda R greater than lambda E}
\end{table}


% % (Avg) lambda_R \geq \lambda_E;  Total travel costs, toll revenue, and Societal cost

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|} 
    \hline
    Weights & Policy &
    \multicolumn{2}{c|}{Travel costs (\$)} & Toll revenue & Societal cost \\
    \cline{3-4}
    $(\lambda_E, \lambda_R, \lambda_I)$ & 
    % (CBCP or DBCP) 
    & \hspace{0.3mm} Eligible \hspace{0.3mm} & Ineligible & (\$) & (\$)  \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(1, 5, 1)$} & CBCP & $1.31 \times 10^4$ & $8.04 \times 10^5$ & $2.65 \times 10^4$ & $6.85 \times 10^5$ \\
    \cline{2-6}
    & DBCP & $1.33 \times 10^4$ & $7.90 \times 10^5$ & $2.79 \times 10^4$ & $6.64 \times 10^5$ \\
    \hline
    \multirow{2}{*}{\centering $(5, 5, 1)$} & CBCP & $1.27 \times 10^4$ & $8.01 \times 10^4$ & $1.86 \times 10^5$ & $7.72 \times 10^5$ \\
    \cline{2-6}
    & DBCP & $1.29 \times 10^4$ & $7.88 \times 10^5$ & $2.25 \times 10^4$ & $7.40 \times 10^5$ \\
    \hline
    \multirow{2}{*}{\centering $(10, 10, 1)$} & CBCP & $1.27 \times 10^4$ & $8.09 \times 10^5$ & $2.04 \times 10^4$ & $7.31 \times 10^5$ \\
    \cline{2-6}
    & DBCP & $1.31 \times 10^4$ & $8.00 \times 10^5$ & $2.47 \times 10^4$ & $6.84 \times 10^5$ \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(5, 1, 1)$} & CBCP & $1.27 \times 10^4$ & $8.01 \times 10^5$ & $1.56 \times 10^4$ & $8.49 \times 10^5$ \\
    \cline{2-6}
    & DBCP & $1.29 \times 10^4$ & $7.71 \times 10^5$ & $7.75 \times 10^3$ & $8.28 \times 10^5$ \\
    \hline 
    \multirow{2}{*}{\centering $(5, 1, 0)$} & CBCP & $1.27 \times 10^4$ & $8.11 \times 10^5$ & $1.73 \times 10^4$ & $4.62 \times 10^4$ \\
    \cline{2-6}
    & DBCP & $1.30 \times 10^4$ & $7.98 \times 10^5$ & $2.09 \times 10^4$ & $4.42 \times 10^4$ \\
    \hline
    \multirow{2}{*}{\centering $(20, 1, 0)$} & CBCP & $1.25 \times 10^4$ & $8.15 \times 10^5$ & $1.61 \times 10^4$ & $2.33 \times 10^5$ \\
    \cline{2-6}
    & DBCP & $1.28 \times 10^4$ & $7.99 \times 10^5$ & $1.89 \times 10^4$ & $2.37 \times 10^5$ \\
    \hline
    \end{tabular}
    \caption{Total travel costs, toll revenues, and societal costs at equilibrium, under the optimal CBCP and DBCP policies with respect to weight parameters $(\lambda_E, \lambda_R, \lambda_I)$ in $S_{\boldlambda}^\paren{1}$, which all satisfy $\lambda_R \geq \lambda_E$.
    }
    % \label{Table: (Avg) Total Travel Costs and Toll Revenue, for lambda R greater than lambda E}
\end{table}




% % (Avg) lambda_R \geq \lambda_E; Societal cost

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|} 
    \hline
    Weights & Policy & Societal cost (\$) \\
    $(\lambda_E, \lambda_R, \lambda_I)$ & 
    % (CBCP or DBCP) 
    & \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(1, 5, 1)$} & CBCP & $6.85 \times 10^5$ \\
    \cline{2-3}
    & DBCP & $6.64 \times 10^5$ \\
    \hline
    \multirow{2}{*}{\centering $(5, 5, 1)$} & CBCP & $7.72 \times 10^5$ \\
    \cline{2-3}
    & DBCP & $7.40 \times 10^5$ \\
    \hline
    \multirow{2}{*}{\centering $(10, 10, 1)$} & CBCP & $7.31 \times 10^5$ \\
    \cline{2-3}
    & DBCP & $6.84 \times 10^5$ \\
    \hline
    \hline
    \multirow{2}{*}{\centering $(5, 1, 1)$} & CBCP & $8.49 \times 10^5$ \\
    \cline{2-3}
    & DBCP & $8.28 \times 10^5$ \\
    \hline 
    \multirow{2}{*}{\centering $(5, 1, 0)$} & CBCP & $4.62 \times 10^4$ \\
    \cline{2-3}
    & DBCP & $4.42 \times 10^4$ \\
    \hline
    \multirow{2}{*}{\centering $(20, 1, 0)$} & CBCP & $2.33 \times 10^5$ \\
    \cline{2-3}
    & DBCP & $2.37 \times 10^5$ \\
    \hline
    \end{tabular}
    \caption{Total travel costs, toll revenues, and societal costs at equilibrium, under the optimal CBCP and DBCP policies with respect to weight parameters $(\lambda_E, \lambda_R, \lambda_I)$ in $S_{\boldlambda}^\paren{1}$, which all satisfy $\lambda_R \geq \lambda_E$.
    }
    % \label{Table: (Avg) Total Travel Costs and Toll Revenue, for lambda R greater than lambda E}
\end{table}


